InsertionNet -- A Scalable Solution for Insertion

Complicated assembly processes can be described as a sequence of two main activities: grasping and insertion. While general grasping solutions are common in industry, insertion is still only applicable to small subsets of problems, mainly ones involving simple shapes in fixed locations and in which the variations are not taken into consideration. Recently, RL approaches with prior knowledge (e.g., LfD or residual policy) have been adopted. However, these approaches might be problematic in contact-rich tasks since interaction might endanger the robot and its equipment. In this paper, we tackled this challenge by formulating the problem as a regression problem. By combining visual and force inputs, we demonstrate that our method can scale to 16 different insertion tasks in less than 10 minutes. The resulting policies are robust to changes in the socket position, orientation or peg color, as well as to small differences in peg shape. Finally, we demonstrate an end-to-end solution for 2 complex assembly tasks with multi-insertion objectives when the assembly board is randomly placed on a table.

==> acknowledgement.tex <==
\section*{Acknowledgment}
% The authors would like to acknowledge support for this project from   Israel Ministry of Science and Technology (2028449).  


==> algorithm.tex <==
{
\SetAlgoNoLine
\begin{algorithm}[!t]
\caption{Backward Learning for Data Collection}\label{Algo:backward}
    \DontPrintSemicolon
    \SetKwFunction{Fupdate}{update\_tree}
    \SetKwFunction{Ftop}{top\_actions}
    \KwIn{Maximum Randomized Location $r_0=10[\textrm{mm}]$; Maximum Randomized Angle $\theta_0=10^\circ$; Maximum Height $z_{\textrm{max}}=50[\textrm{mm}]$; Force threshold $F_{\textrm{th}}$; Momentum threshold $M_{\textrm{th}}$}
    \textbf{Init:} Insert peg/plug into the hole, register final pose $L$ \\
    \textbf{Set:} $(x_0,y_0,z_0, \theta_{x0}, \theta_{y0}, \theta_{z0})=L$ \\
    \textbf{Init:} Initialize buffer $B=\emptyset$ \\
    \For{$i \leftarrow 1,\ldots,N_p$}
    {
        \tikzmk{A}
        $x^i \sim \textrm{Uniform}[x_0-r_0, x_0+r_0] \quad \quad \quad $ \textbf{Generates}\\
        $y^i \sim \textrm{Uniform}[y_0-r_0, y_0+r_0] \quad \quad \quad \quad$  \textbf{Target T} \\
        $\theta^i_{x},\theta^i_{y},\theta^i_{z} \sim \textrm{Uniform}[-\theta_0, \theta_0]$ \\
        Set robot to state $(x_0,y_0,z_0+z_{\textrm{max}}, \theta_{x0}, \theta_{y0}, \theta_{z0})$ \\
        Set target $T=(x^i,y^i,z_o, \theta^i_{x},\theta^i_{y},\theta^i_{z})$ \\
        \tikzmk{B}
        \boxit{blue}
        Move Robot to $T$ \\ 
        \While{Robot did not reach $T$} {
            Measure force $F_i=(f_x, f_y, f_z)$ \\
            Measure moment $M_i=(m_x, m_y, m_z)$ \\
            \If{$F_i \ge F_\textrm{th}$ or $M_i \ge M_\textrm{th}$} {
                $D_i = \{x^i , y^i , z^i, \theta^i_{x}, \theta^i_{y}, \theta^i_{x}\}$ \\
                Capture $\textrm{Img}_i$ from $45^\circ$ camera \\
                $\textrm{Obs}_i = \{ \textrm{Img}_i, F_i, M_i \}$ \\
                $\textrm{Action}_i = \{L-D_i\}$ \\
                Append $\{\textrm{Obs}_i, \textrm{Action}_i\}$ to $B$ \\
                %break while loop \\
           }        
        }
    }
    \Return $B$ \\
\end{algorithm}

}


==> into_check.tex <==
\section{Introduction}
Even in routine tasks such as inserting a car key into the
ignition, humans effortlessly combine the senses of vision
and touch to complete the task. Visual feedback provides semantic and geometric object properties for accurate reaching
or grasp pre-shaping. Haptic feedback provides observations
of current contact conditions between object and environment
for accurate localization and control under occlusions. These
two feedback modalities are complementary and concurrent
during contact-rich manipulation [8]. Yet, there are few
algorithms that endow robots with a similar ability. While
the utility of multimodal data has frequently been shown in
robotics [7, 45, 48, 54], the proposed manipulation strategies
are often task-specific. While learning-based methods do not
require manual task specification, the majority of learned
manipulation policies close the control loop around a single
modality, often vision [15, 21, 34, 58].
In this work, we equip a robot with a policy that leverages
multimodal feedback from vision and touch, two modalities
with very different dimensions, frequencies, and characteristics. This policy is learned through self-supervision and
generalizes over variations of the same contact-rich manipulation task in geometry, configurations, and clearances. It
is also robust to external perturbations. Our approach starts
with using neural networks to learn a shared representation
of haptic and visual sensory data, as well as proprioceptive data. Using a self-supervised learning objective, this
network is trained to predict optical flow, whether contact
will be made in the next control cycle, and concurrency of
visual and haptic data. The training is action-conditional to
encourage the encoding of action-related information. The
resulting compact representation of the high-dimensional and
heterogeneous data is the input to a policy for contact-rich
manipulation tasks using deep reinforcement learning. The
proposed decoupling of state estimation and control achieves
practical sample efficiency for learning both representation
and policy on a real robot. Our primary contributions are:

==> task_description.tex <==
\section{TASK DESCRIPTION}
\label{sec:GeneralInsertion}
Our primary objective in this work is to develop an algorithm that is directly applicable to as many real-world insertion tasks as possible. In this section, we elaborate on what a \emph{general insertion solution} means. \\
\textbf{Scalability:} A general solution should be able scale to different peg-in-a-hole, plug insertion, and threading problems, etc. The solution should be able to simultaneously solve all these use-cases with a single pre-trained policy. \\
\textbf{Size Independence:} The peg and the hole size can vary between different assembly applications, from avionic to micro-electronic products. A general algorithm should not be size dependent. \\
\textbf{Unfixed Grasping:}  In many of the currently available solutions, the grasping aspect of the problem is ignored by fixing the plug to the EEF. In our case, accidental peg slips and limited manipulation is considered and learned. \\
\textbf{Location:} The ability to insert the same peg repeatedly in different locations is necessary in many industrial applications, such as electrical panel assembly. Therefore, it is required that an algorithm operate in any given location or orientation without additional learning. \\
\textbf{Color Independence:} Changing the color of a plug or socket should not result in failure. \\
\textbf{Transfer Learning Capabilities:} The algorithm should be able to share information between different insertion tasks. Therefore, training a new insertion task should require less data than learning the task from scratch.

